Main-sequence systems: orbital stability in stellar binaries

The majority of star formation results in binaries or higher multiple systems, and planets in such systems are constrained to a limited range of orbital parameters in order to remain stable against perturbations from stellar companions. Many planets have been discovered in such multiple systems (such as stellar binaries), and understanding their stability is important in exoplanet searches and characterization. In this chapter, we focus on the orbital stability of planets in stellar binaries. We review key results based on semi-analytical secular (long term) methods, as well as results based on N-body simulations and more recent Machine Learning methods. We discuss planets orbiting one of the stellar binary components (S-type) and those orbiting both stars (P-type) separately.

==> binary_rebuttal.tex <==
***Section 4
----1st paragraph: Would be helpful to mention the frequencies/number of
known planets in S-type and P-type systems.

There are only ~20 known P-type planets, which potentially have their own observational biases for/against detection.  We added an approximate percentage of the known planets in binaries that are P-type, where readers can follow the link to Richard Schwarz’s online database to find precise (and updated) counts.

***Fig. 7
----The caption states that the most massive component is m_1. Is m_1
always greater than m_3 here?

It doesn’t have to be the case, but most of the S-type planets are detected around the more massive star of a stellar binary, where there are observational biases for this, mostly due to the brightness differences between the stars and the faintness limit for performing radial velocity measurements.  Since our section is focused on the stability and dynamics, it seems that this point would be outside the current scope.

***Section 4.1
----1st paragraph, 2nd sentence: did you mean m_1 ~ m_3 instead of m_1 ~
m_2?

This was corrected to m_3, where we thank the reviewer for pointing out this typo.

***Section 4.1.1
----Eqs. (9-10): It would be helpful to explain why we break up
eccentricity in this way and the importance of defining alpha to
quantify hierarchy.

Gongjie, isn’t this comment more relevant to Hareesh’s section?  Could we just refer to his description?

----I think Eq. (15) should appear immediately after Eq. 12. Otherwise,
readers could be puzzled and/or think that these variables were
previously introduced.

Rearranging the equations causes a lot of definitional problems later in the text, where we have added a short description of the constants in terms of the mathematics.  The full definition of these constants in Eq. (15) gives their physical meaning.

----Paragraph after Eq. (16): the sentence "Each of the three initial
conditions have the same value for epsilon_H and g_H" I think is
confusingly worded.

We thank the reviewer for pointing this out, where we reworded this sentence to emphasize that the e_free largely determines the amplitude of variation.

----Right before Eq. (21), "can be finite sum" --> "can be represented
as a finite sum"

This has been corrected.

***Section 4.1.2
----2nd paragraph: "where we may" --> "whereas we may"

This has been corrected.

----3rd paragraph: "match with an accuracy less than 0.5%" --> "match
with an accuracy more than 99.5%"

This has been corrected.

----5th paragraph: Would it be less confusing to use e_{free} rather
than [e_{max} - e_F]? Also, perhaps adding a sentence like the following
would be helpful: "The goodness of the analytical approaches depends on
how well the solid lines match the dots."

No, using e_free would not be accurate.  We initially used e_free, but then realized the confusion.  The data points are produced via n-body simulations which contain more than just the secular interaction.  The difference of measured e_max with e_F shows how the secular approximation breaks down as a planet enters a region dominated by N:1 MMRs.

We added the proposed sentence to this paragraph.

----6th paragraph: "more dire" means what specifically?

We edited the sentence to use more precise language.

----7th paragraph: I don't see any grey region on the figure. Also,
words are missing when describing the red dots and blue dots later in
the paragraph.

We added a qualifying statement that more strongly hints our use of language.  Here “grey” does not refer to color specifically, rather how the term is used in other contexts where the determination of stability is ambiguous (i.e., grey).  This sets up the usage later made specifically by Dvorak.

We added more context around what the simulations with red or blue dots represent.

***Fig. 11
----I think the colour in the top axis is too light. Why not write that
in black?

We chose the color here to emphasize the difference in axis labels between Figs. 10 and 11.  The top axis did not exist in the original figure (Quarles et al. 2018a), where we opted to keep the bottom axis to better match the reference content.  Cyan is within the standard color scheme, where it is a contrasting color to the red and a significantly different hue compared to the blue that exists within Fig. 11.

----I think the colours for the eccentric and "both stable" systems are
too similar.

The color for both stable (purple) reflects that it occupies the intersection of eccentric (red) and circular (blue) categories.

----I think the meaning of the lack of dots between the 19:1 and 22:1 in
the upper panel should be stated.

There isn’t a lack of dots in this area, where there is an overlap between the two categories.  This is why the color is purple following the color scheme given in the bottom panel.

***Section 4.1.3
----1st paragraph, 2nd sentence: "that this occurs"... what is "this"?

The “this” refers to the limitations in the secular approximations stated in the previous sentence.  We modified the language to “the limitations become evident” to be more precise.

Also, "Eq. 14 break down" --> "Eq. 14 can break down"

This should have been a reference to Eq. 15, which has been corrected.  The helper verb “can” has been added as suggested, although the language editors may remove it later.

----2nd paragraph: "where becomes more natural" --> "where it becomes
more natural"

This has been corrected.

----3rd paragraph: Why should C_1 limit planetary stability?

C_1 corresponds to using the distance to L_1 within \alpha in Eq. 24.  L_1 is an unstable point within the potential.  Therefore, Jacobi constants that approach C_1 should represent a transition to instability.  This sentence has been modified to convey this additional context.

----5th paragraph: Are there too many references in the set from
1979-1983? Recall that the nominal reference limit is 30.

Gongjie, I think we are way beyond 30 references.  What does cutting 2-3 matter here?

----Right before Eq. (25) perhaps write out alpha_c as = a_c/a_{bin}
without using /frac.

This has been corrected.

----The whole Pg. 18 is quite interesting and includes a good history
and comparison.

***Figs. 9-18
----In the caption of each, specify if the system is S-type or P-type.
This has been added to each caption.

****Eqs. (26), (39), (40)
----Might want to note how they simplify when e_{bin} = 0 to produce
rule-of-thumbs, especially even when mu^{cross} = 0.5.

This approach is not helpful in practice because nearly all planets in binaries exist in either eccentric binaries or binaries of unknown eccentricity.  The fitting formulas are presented for historical purposes, where modern computing techniques (grid interpolation or DNN) are much more useful and accurate.

****Pg. 19
----The listing of the 6 assumptions is great.

****Fig. 14
----State in caption that the angles are given in degrees.
This has been added.

****Section 4.2
----Would it be helpful to draw two side-by-side cartoons to visually
show readers the difference between S-type and P-type systems?

****Section 4.2.1
----Eq. (28): specify if this disturbing function is truncated according
to either eccentricity.
We added a sentence noting that the approximation level applied here is the same as the one applied in the S-Type planet case.

----Paragraph after Eq. (35): wording makes it slightly unclear if
epsilon_{mn} = 0 is realistic or not when e_{bin} = 0 or mu^{cross} =
0.5. Perhaps be more direct.

We are not sure what is meant here.  We describe that the secular approximation epsilon does not match the N-body simulation and point to a reference if a reader wants to see the next-leading order approximation.

****Pg. 22
----You use e_{mn} here and not epsilon_{mn}, in contrast to the
previous page.

This has been made consistent.

----Right before Eq. (36), "eff" --> "e_{ff}"

This has been corrected.

----Right after Eq. (37), what is "e_F"?

It is the forced eccentricity. We added a descriptor to make this more clear.

****Pg. 23
----"we would expect from vector addition" refers to which equation?

It does not refer to a specific equation, but a mathematical principle.  This has been modified to be more clear.

****Pg. 25
----"(Eq. 39 or 40" needs a closing parenthesis.

This has been corrected.

